Flow Equilibria via Online Surge Pricing

We explore issues of dynamic supply and demand in ride sharing services such as Lyft and Uber, where demand fluctuates over time and geographic location. We seek to maximize social welfare which depends on taxicab and passenger locations, passenger valuations for service, and the distances between taxicabs and passengers. Our only means of control is to set surge prices, then taxicabs and passengers maximize their utilities subject to these prices. We study two related models: a continuous passenger-taxicab setting, similar to the Wardrop model, and a discrete passenger-taxicab setting. In the continuous setting, every location is occupied by a set of infinitesimal strategic taxicabs and a set of infinitesimal non-strategic passengers. In the discrete setting every location is occupied by a set of strategic agents, taxicabs and passengers, passengers have differing values for service. We expand the continuous model to a time-dependent setting and study the corresponding online environment. Surge prices are in passenger-taxicab equilibrium if there exists a min cost flow that moves taxicabs about such that (a) every taxicab follows a best response, (b) all strategic passengers at $v$ with value above the surge price $r_v$ for $v$, are served and (c) no strategic passengers with value below $r_v$ are served (non-strategic infinitesimal passengers are always served). This paper computes surge prices such that resulting passenger-taxicab equilibrium maximizes social welfare, and the computation of such surge prices is in poly time. Moreover, it is a dominant strategy for passengers to reveal their true values. We seek to maximize social welfare in the online environment, and derive tight competitive ratio bounds to this end. Our online algorithms make use of the surge prices computed over time and geographic location, inducing successive passenger-taxicab equilibria.

==> figures.tex <==


\begin{figure}
\vbox{\hbox{
\begin{minipage}{0.49\textwidth}
\centering
\begin{tikzpicture}[shorten >=1pt, auto, node distance=3cm, ultra thick,
node_style/.style={circle,draw=blue,fill=blue!20!,font=\sffamily\Large\bfseries},
edge_style/.style={draw=black, ultra thick},scale=0.7]

\node[node_style] (v1) at (-4,2) {$v_1$}; \node[node_style] (v2) at
(0,2) {$v_2$}; \node[node_style] (v3) at (4,2) {$v_3$};
\node[node_style] (v4) at (-4,-2) {$v_4$}; \node[node_style] (v5) at
(0,-2) {$v_5$}; \node[node_style] (v6) at (4,-2) {$v_6$};

\draw[edge_style] (v1) edge node{1} (v2); \draw[edge_style] (v2)
edge node{1} (v3); \draw[edge_style] (v4) edge node{1} (v5);
\draw[edge_style] (v5) edge node{1} (v6); \draw[edge_style] (v1)
edge[bend left] node{2} (v3); \draw[edge_style] (v4) edge[bend
right] node{2} (v6);

\draw[edge_style] (v1) edge node[near start]{1} (v4);
\draw[edge_style] (v5) edge node[near end]{2} (v1);
\draw[edge_style] (v1) edge node[very near start]{3} (v6);

\draw[edge_style] (v4) edge node[very near end]{2} (v2);
\draw[edge_style] (v2) edge node[near start]{1} (v5);
\draw[edge_style] (v2) edge node[very near start]{2} (v6);

\draw[edge_style] (v4) edge node[very near end]{3} (v3);
\draw[edge_style] (v3) edge node[near start]{2} (v5);
\draw[edge_style] (v3) edge node[near start]{1} (v6);

\end{tikzpicture}

\captionof{figure}{Example road network, with costs along
edges.} \label{fig:example}\end{minipage}

\begin{minipage}{0.49\textwidth}
\centering
\begin{tikzpicture}[shorten >=1pt, auto, node distance=3cm, ultra thick,
node_style/.style={circle,draw=blue,fill=blue!20!,font=\sffamily\Large\bfseries},
edge_style/.style={draw=black, ultra thick},
dedge_style/.style={->,> = latex}, scale=0.6]


\node[node_style] (v1) at (-4,2) {$v_1$}; \node[node_style] (v2) at
(0,2) {$v_2$}; \node[node_style] (v3) at (4,2) {$v_3$};
\node[node_style] (v4) at (-4,-2) {$v_4$}; \node[node_style] (v5) at
(0,-2) {$v_5$}; \node[node_style] (v6) at (4,-2) {$v_6$};

\draw[dedge_style] (v3) edge[loop right] node{$\frac{1}{8}$} (v3);
\draw[dedge_style] (v3) edge node[near start]{$\frac{1}{8}$} (v6);
\draw[dedge_style] (v3) edge node[near start]{$\frac{1}{12}$} (v5);

\draw[dedge_style] (v2) edge node[near start]{$\frac{7}{24}$} (v5);
\draw[dedge_style] (v2) edge node[near
start,left=10pt]{$\frac{1}{24}$} (v4);

\draw[dedge_style] (v1) edge node[near start,left]{$\frac{1}{3}$}
(v4);

\end{tikzpicture}
\captionof{figure}{A min earthmover cost flow from supply vector
$s^{t-1}=\langle\frac{1}{3},\frac{1}{3},\frac{1}{3},0,0,0\rangle$ to
demand vector
$d^t=\langle0,0,\frac{1}{8},\frac{3}{8},\frac{3}{8},\frac{1}{8}\rangle$.}
\label{fig:flow1}
\end{minipage}
} \hbox{
\begin{minipage}{0.49\textwidth}
\centering
\begin{tikzpicture}[shorten >=1pt, auto, node distance=3cm, ultra thick,
node_style/.style={circle,draw=blue,fill=blue!20!,font=\sffamily\Large\bfseries},
edge_style/.style={draw=black, ultra thick},
dedge_style/.style={->,> = latex},scale=0.6]


\node[node_style] (v1) at (-4,2) {$v_1$}; \node[node_style] (v2) at
(0,2) {$v_2$}; \node[node_style] (v3) at (4,2) {$v_3$};
\node[node_style] (v4) at (-4,-2) {$v_4$}; \node[node_style] (v5) at
(0,-2) {$v_5$}; \node[node_style] (v6) at (4,-2) {$v_6$};

\draw[dedge_style] (v3) edge[loop right] node{$\frac{1}{8}$} (v3);
\draw[dedge_style] (v3) edge node[near start]{$\frac{1}{8}$} (v6);
\draw[dedge_style] (v3) edge node[near start]{$\frac{1}{24}$} (v5);
\draw[dedge_style] (v3) edge node[near start, above]{$\frac{1}{24}$}
(v4);

\draw[dedge_style] (v2) edge node[near start]{$\frac{1}{3}$} (v5);

\draw[dedge_style] (v1) edge node[near start, left]{$\frac{1}{3}$}
(v4);

\end{tikzpicture}
\captionof{figure}{Another min earthmover cost flow from from supply
vector
$s^{t-1}=\langle\frac{1}{3},\frac{1}{3},\frac{1}{3},0,0,0\rangle$ to
demand vector
$d^t=\langle0,0,\frac{1}{8},\frac{3}{8},\frac{3}{8},\frac{1}{8}\rangle$.}
\label{fig:flow2}
\end{minipage}}}
\end{figure}


\begin{figure}\centering
\hbox{\begin{minipage}{0.49\textwidth} \centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
            \hline
            &  $m_{14}$&  $m_{24}$&  $m_{25}$&  $m_{33}$&  $m_{35}$&  $m_{36}$\\
            \hline
            $b_{14}$&  3&  3&  2&  2&  2&  1\\
            \hline
            $b_{24}$&  2&  2&  3&  3&  3&  2\\
            \hline
            $b_{25}$&  2&  2&  3&  3&  3&  2\\
            \hline
            $b_{33}$&  1&  1&  2&  4&  2&  3\\
            \hline
            $b_{35}$&  1&  1&  2&  4&  2&  3\\
            \hline
            $b_{36}$&  1&  1&  2&  4&  2&  3\\
            \hline
            $p_{ij}$&  0&  0&  1&  3&  1&  2\\
            \hline
        \end{tabular}
            \captionof{figure}{Item valuations for bidders $B^f=\{b_{14},b_{24},b_{25},b_{33},b_{35},b_{36}\}$, items $M^f=\{m_{14},m_{24},m_{25},m_{33}, m_{35},m_{36}\}$, where $f$ is the min earthmover flow given in Figure \ref{fig:flow1}. Note that in Figure \ref{fig:example} we have $\max_{ij}\left(\ell_{ij}\right)=3$ and thus $C=4$. The last row gives Walrasian market clearing prices for items $m_{ij}$. Note that $p_{ij}=p_{ij'}$ for all $b_{ij}, b_{ij'}\in B^f$. }
    \label{fig:marketfig}
\end{minipage}
\quad
\begin{minipage}{0.49\textwidth}
\centering
        \begin{tabular}{|c|c|c|c|c|c|c|}
            \hline
            &  $v_1$&  $v_2$&  $v_3$&  $v_4$&  $v_5$&  $v_6$\\
            \hline
            $r^t_i$&  1&1&1&4&3&2\\
            \hline

        \end{tabular}
            \captionof{figure}{Surge prices resulting in a flow-equilibrium with $s^t=d^t$. These surge price for $v_j$ is $C-p_{ij}$ if there exists some bidder $b_{ij}\in B^f$ and 1 otherwise. The Walrasian prices $p_{ij}$ appear in Figure \ref{fig:marketfig}. }
    \label{fig:surgeprice}
\end{minipage}
}
\end{figure}


==> results.tex <==

\begin{center}
\begin{figure}\begin{center}
{\renewcommand{\arraystretch}{1.3}% for the vertical padding
\begin{tabular}{|l|l|l|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  &\begin{tabular}{l}
     Bound on max demand \\
     $d_i^t\leq 1/\rho$ for all $i$,$t$
   \end{tabular}      & \begin{tabular}{l} As function of total drift\\ $\delta = \frac{1}{T} \cdot \sum_{t=1}^T \sum_{i=1}^k \frac{|d^t_i - d^{t-1}_i|}{2}$\\ ($0\leq \delta \leq 1$)\end{tabular} \\ \hline
  $\ell_{ij}>1$ & \begin{tabular}{l} $\frac{\rho}{k} \leq \mathrm{c.r.} \leq \frac{\rho}{k}\cdot\frac{\ell^2_{\max}}{\ell_{\max}-1}$ \\(Theorem \ref{thm:arbitrary})\end{tabular}& \begin{tabular}{l}$1-\delta\ell_{\max}\leq \mathrm{c.r.}$ \\ (Theorem \ref{?}) \end{tabular} \\ \hline
  $\ell_{ij}=1$ & \begin{tabular}{l} $\sqrt{\frac{\rho}{k}}$ \\ (Theorem \ref{thm:ellij1})\end{tabular} & \begin{tabular}{l} $1-\delta \leq \mathrm{c.r.} \leq 1-\frac{\delta}{6}$ \\(Theorem \ref{?})\end{tabular} \\
  \hline
\end{tabular}}\end{center}
  \caption{Competitive ratios for the surge control online algorithm in different scenarios.}
\end{figure}
\end{center}

\subsection{Using Surge Pricing to Control Supply}

%We first study how surge pricing can be used so that desired
%supplies arise as Nash equilibria, see Section \ref{sct:surge}. The
%first result shows how to change supply at time $t$ to meet demand
%at time $t+1$. The reason this is not trivial is because of the
%distances that need to be covered (paid for) by the suppliers, so the
%surge pricing has to compensate the suppliers for the extra distance.
%We reduce this to a problem of competitive market equilibrium.


%Consider a flow function $f:V\times V$ that redistributes supply from time step $t-1$,
% Let $s^{t-1}=\langle s^{t-1}_1, \ldots, s^{t-1}_k \rangle$ be the supply at time $t-1$,  $d^{t}=\langle d^{t}_1, \ldots, d^{t}_k \rangle$ the demand at time $t$, and $s^{t}=\langle s^{t}_1, \ldots, s^{}_k \rangle$ the supply at time $t$. Furthermore, let $r^t=\langle r^t_1,\ldots,r^t_k\rangle$ be the surge price vector at time $t$. Then, the utility of moving from vertex $x$ to vertex $y$ at time $t$, $\mu^t(x\rightarrow y)$, is defined as
%$$\mu^t(x\rightarrow y)=\left(r^t_y\right)\cdot\min\left(1,{d^t_y}/{s^t_y}\right)-\ell_{xy}.$$
%
%
%    We define a flow function as being in equilibrium for $s^{t-1}$,$s^t$,$d^t$ and $r^t$ if for all $w,x,y\in V$ whenever $f(x,y)>0$ {\sl i.e. there is flow from $x$ to $y$} then $\mu^t(x\rightarrow y)\geq\mu^t(x\rightarrow w)$.



%\begin{theorem}\label{thm:surge}
%  Given a set of distances $\ell_{ij}$ and arbitrary supply vector at time $t-1$, $s^{t-1}=\langle s^{t-1}_1, \ldots, s^{t-1}_k \rangle$. Let the demand vector at time $t$ be $d^t=\langle d^t_1, \ldots, d^t_k\rangle$. Then, there exists a surge price vector $r^t=\langle r^t_1,\ldots,r^t_k\rangle$
%that results in a Nash Equilibrium where $s^t=d^t$. Moreover, this
%Nash Equilibrium is unique.
%\end{theorem}
%
%It will be useful to consider the following special case:
%
%\begin{corollary}
%    For the special case where $\ell_{ij}=1$ for all $i,j$, the surge pricing that induces $s^t=d^t$ is particularly simple and sets $$r^t = \left\{\begin{array}{cl}
%    r^t_i=1 & \mbox{\rm When $d^t_i\leq s^{t-1}_i$} \\
%    r^t_i=2 & \mbox{\rm When $d^t_i>s^{t-1}_i$}
%    \end{array}\right..$$
%\end{corollary}

%We next show that any supply profile can be achieved as a flow
%equilibrium, with the restriction that the total target supply is
%equal to the total original supply, and that the target supply is
%equal to zero on vertices where the demand is zero.
%
%\begin{theorem}
%    Given a set of distances $\ell_{ij}$ and arbitrary supply at time $t-1$. Let the demand vector at time $t-1$ $d^t=\langle d^t_1, \ldots, d^t_k \rangle$. Consider an arbitrary target vector $h^t=\langle h^t_1, \ldots, h^t_k\rangle$, where $h^t_i=0$ if $d^t_i=0$, and $\sum_{i=1}^k h^t_i =1$. Then, there exists a surge price vector $r^t=\langle r^t_1, \ldots, r^t_k\rangle$ so that the target vector $h^t$ can be realized as the supply in a Nash Equilibrium.
%\end{theorem}


%\subsection{Maximizing Social Welfare}
%
%Next, we turn to maximizing social welfare via surge pricing. Recall
%that this is defined to be the fraction of requests served minus the
%transportation cost (the earthmover distance from the old supply
%vector to the new supply vector).
%
%The algorithms are viewed as online algorithms that simply set the
%supply at time $t+1$, ignoring individual incentives. However, all
%of the algorithms presented can be viewed as simply setting surge
%prices rather than an online algorithm that determines the next
%supply vector by fiat. This follows from Theorem \ref{thm:surge}
%described above.
%
%We consider how the competitive ratio depends on properties of the
%input sequence: \begin{itemize} \item When the max demand on any vertex is bounded by $1/\rho \leq 1$, $d_i^t \leq 1/\rho$ for all $i$, $t$. For $\rho=1$ then there are no restrictions on the demand.
%\item When the average $L_1$ distance
%between successive demand vectors is bounded. {\sl I.e.}, as a function of the average $L_1$ distance, $\delta$, where $$\delta=\sum_{t=1}^T\sum_{i=1}^k |d^t_i-d^{t-1}_i|/(2T).$$ \end{itemize}
%
%As we normalize the sum of demands to one, a small bound on the max demand translates into the statement that no geographic locale ever becomes the dominant demand vertex. Bounding the average $L_1$ distance between demand vectors says that, on average, the changes in demand are not that dramatic. 
%
%Our results are give as a function of these two sequence parameters, because these may be more ``realistic" non-worst case assumptions, and the results are better when the max demand is small or when the average drift is small. That said, the most interesting and strongest result is when the max demand and average drift are arbitrary, and is given simply by assuming $\rho=1$ and no assumptions on drift. 
%
%We deal separately with restrictions on max demand and on the drift. Moreover, for max demand we assume that it is known, however this is not required and we discuss how to avoid this dependency later. In both cases we distinguish between the case where
%$\ell_{ij}$ is unrestricted and when $\ell_{ij}=1$.
%
%We first show the following:
%\begin{theorem} \label{thm:arbitrary}
%    The competitive ratio of the general problem (no restrictions on drift, max demand, or distances) is $\Theta(\frac{1}{k})$.
%\end{theorem}
%
%Lemma \ref{lem:lessimmediate} shows that if $\ell_{ij}>1$ for all $1 \leq i\leq j \leq k$ then this result cannot be improved, {\sl i.e.}, cannot be better than
%$O(\frac{1}{k})$, Lemma \ref{lem:immediate} is immediate and shows
%that a competitive ratio of $1/k$ is trivially achievable.
%
%\begin{lemma}\label{lem:lessimmediate}
%  For every $\epsilon > 0$, assume that $\ell_{ij}=1+\epsilon$ for all $1 \leq i\leq j \leq k$. Then no online algorithm can guarantee a social welfare greater than $(1/k)\cdot\frac{(1+\epsilon)^2}{k\cdot\epsilon}$ of the optimal social welfare. For any fixed $\epsilon>0$ this bound is $O(1/k)$. The adversarial sequence used to derive this bound has unbounded drift.
%\end{lemma}
%
%\begin{lemma}\label{lem:immediate}
%  For any $\ell_{ij}$, $1\leq i\leq j\leq k$, and any drift $\delta$, a trivial randomized online algorithm (move all supply to a random vertex) has a competitive ratio $= \frac{1}{k}$.
%\end{lemma}
%
%Theorem \ref{thm:ellij1} considers the case where all distances
%$\ell_{ij}=1$, and assumes no other restrictions on the demand
%sequence. In this case the competitive ratio improves to
%$\Theta(\frac{1}{\sqrt{k}})$.
%
%\begin{theorem}\label{thm:ellij1}
%    Fix $k\geq 2$, and let $\ell_{ij}=1$ for all $1\leq i\leq j\leq k$, furthermore allow unrestricted drift and unrestricted max demand in the demand sequence. Then, the competitive ratio is $\Theta(\frac{1}{\sqrt{k}})$.
%\end{theorem}
%
%The proof of Theorem \ref{thm:ellij1} follows from the following two
%lemmata, Lemma \ref{lem:ellij1} and Lemma \ref{lem:ellij2}.
%
%\begin{lemma}\label{lem:ellij1}
%Consider an adversary that chooses $c^t_i\in K$ uniformly at random
%at time $t$, and sets the demand $d^t_i=1$ and $d^t_j=0$ for all
%$j\neq i$. Any online algorithm has expected social welfare equal to
%$\frac{T}{k}$, the optimal offline algorithm has expected social
%welfare of at least $\Theta(\frac{T}{\sqrt{k}})$.
%  \end{lemma}
%
%\begin{lemma}\label{lem:ellij2}
%  There exists an online algorithm $A$ such that for any sequence $\overline{d}$ of demand vectors, such that the competitive ratio, $A(\overline{d})/OPT(\overline{d}) \geq O(1)/\sqrt{k}.$
%\end{lemma}
%
%
%
%%\begin{theorem}
%%   Let $Q_\rho=\{\overline{d} | OPT(\overline{d}) \geq \rho |\overline{d}|\}$, {\sl i.e.}, $Q_\rho$ is a collection of sequences for which OPT gains at least $\rho$ social welfare on average per time step. There is an online algorithm $A_\rho$ for which $A_\rho(\overline{d}) >\rho^2\cdot |\overline{d}|$ for all $\overline{d}\in Q_\rho$.
%%\end{theorem}
%
%Let $\delta$ be an upper bound on the average drift, {\sl i.e.}, the
%average $L_1$ distance between successive demand vectors, the next
%theorem gives a competitive ratio of $(1-\delta)$ when all distances
%are one:
%
%\begin{theorem}
%    Let $\ell_{ij}=1$ for all $i,j$. Then for some $0<\delta\leq1$ the trivial algorithm that sets $s^t=d^t$ for all $t$ is ($1-\delta$)-competitive.
%\end{theorem}
%
%\begin{theorem}
%    Let $\ell_{ij}=1$ for all $i,j$. Then for any $0<\delta\leq1$ no online algorithm can be better that ($1-\frac{\delta}{6}$)-competitive.
%\end{theorem}
%
%
%\begin{theorem}
%    For any $0<\delta\leq1$ the trivial online algorithm that sets $s^t_i=d^t_i$ is $(1-\delta\cdot\ell_{\max})$-competitive.
%\end{theorem}

